A container-based facility for testing 20'000 20-inch PMTs for JUNO

The main goal of the JUNO experiment is the determination of the neutrino mass ordering. To achieve this, an extraordinary energy resolution of at least $3\,\%$ at $1\,$MeV is required for which all parts of the JUNO detector need to meet certain quality criteria. This is relevant in particular for those which are related to the energy resolution of the detector, such as the photomultiplier tubes (PMTs) to be deployed in JUNO. This paper presents the setup and performance of a dedicated PMT mass testing facility to examine and characterize the performance of the 20-inch JUNO PMTs. Its quasi-industrial size and operation level allows to test all 20000 PMTs intended to be used in the JUNO experiment. With this PMT mass testing system, several key characteristics like dark count rate, peak-to-valley ratio, photon detection efficiency, and timing resolution have been determined at an operating gain of $1\times10^7$ and assessed with respect to the requirements of JUNO. Measurement conditions and modes for the PMTs as well as estimated accuracies for the determination of the individual PMT parameters with the system are presented as well.

==> packages.tex <==
\usepackage{lmodern}
\usepackage{etoolbox}

\usepackage[ngerman,english]{babel}		   	% Sprache: deutsch + englisch
%\usepackage{german,a4}		               	% Sprache: deutsch
\usepackage[ansinew]{inputenc}		       	% Umlaute
\usepackage[T1]{fontenc}	               	% Worttrennung von Woertern mit Umlauten
\usepackage{graphicx}		               	% für Bilder
\usepackage{tabularx}						% für Tabellen
\usepackage{tabulary}						% für Tabellen
%\usepackage[hang]{subfigure}					% mehr Bilder
\usepackage{amsmath,amssymb}             	% für Formeln
\usepackage{endnotes}						% für Fussnoten
\usepackage{footmisc}						% Fußnotenoptionen
\usepackage{here}                         	% Positionen erzwingen
\usepackage[font=small, labelfont=bf, format=plain, indention=0.5cm]{caption} % Bildunterschriften-Optionen
\usepackage{fancyhdr}						% für Kopzeile
\usepackage{xcolor}							% für farbigen Text
\usepackage[inner=2.5cm, outer=2.5cm, top=3cm, bottom=4cm]{geometry} % Seitenränder-Optionen
\usepackage{booktabs}						% für Tabellen
\usepackage{isotope}	      				% für Darstellung von Isotopen
\usepackage{url}							% für Websiten
\usepackage[numbers,sort&compress]{natbib}	% [numbers][authoryear] Für Literaturverzeichnis
\usepackage{wrapfig}						% für Grafiken im Fließtext
\usepackage{multirow}						% für Zeilenzusammenschlüsse in Tabellen
\usepackage{setspace}						% für Zeilenabstand-Einstellungen
\usepackage{alltt}							% für verbatim-Umgebung mit Befehlen
\usepackage{acronym}						% für Abkürzungen
\usepackage{hyperref} 						% für Hyperlinks in Verweisen und Zitaten
%\usepackage{hypernat}
\usepackage{bbold}							% for unit matrix symbol \mathbb{1}
%\usepackage[clearempty]{titlesec}
%\usepackage[style=alphabetic]{biblatex}	% Literaturverzeichnis Zusatz
%\usepackage{luximono}
%\bibpunct[, ]{[}{]}{;}{a}{,}{,}

\usepackage{pstricks}
\usepackage{braket}
\usepackage{bookmark}
\usepackage{longtable}
\usepackage{latexsym} 
\usepackage{makeidx}
\usepackage{textcomp}
\usepackage{colordvi}
%\usepackage{subfig}
%\usepackage{floatfig}
\usepackage{enumitem}

\usepackage{wasysym} %\permil
\usepackage{excludeonly}
\usepackage{array}
%\usepackage{breqn}
\usepackage{mathtools}

\usepackage{nicefrac}

\usepackage{dsfont}
\usepackage{empheq}

\usepackage{siunitx}



